Class-Specific Semantic Reconstruction for Open Set Recognition

Open set recognition enables deep neural networks (DNNs) to identify samples of unknown classes, while maintaining high classification accuracy on samples of known classes. Existing methods basing on auto-encoder (AE) and prototype learning show great potential in handling this challenging task. In this study, we propose a novel method, called Class-Specific Semantic Reconstruction (CSSR), that integrates the power of AE and prototype learning. Specifically, CSSR replaces prototype points with manifolds represented by class-specific AEs. Unlike conventional prototype-based methods, CSSR models each known class on an individual AE manifold, and measures class belongingness through AE's reconstruction error. Class-specific AEs are plugged into the top of the DNN backbone and reconstruct the semantic representations learned by the DNN instead of the raw image. Through end-to-end learning, the DNN and the AEs boost each other to learn both discriminative and representative information. The results of experiments conducted on multiple datasets show that the proposed method achieves outstanding performance in both close and open set recognition and is sufficiently simple and flexible to incorporate into existing frameworks.

==> content_revision/section2.tex <==
\section{Related Work}
% The methods for open set recognition can be roughly divided into two categories, traditional methods and deep learning-based methods. 

Our work is mainly related to open set recognition, particularly AE-based methods and prototype-like methods. Open set recognition is naturally related to some other problems (\eg out-of-distribution (OOD) detection \cite{hendrycks2016a} and novelty detection \cite{perera2019ocgan}, etc). The OOD detection methods are briefly discussed in this section.

\subsection{Open Set Recognition}

Traditional machine learning methods leverage the scores produced by the classifiers, the unknown samples can be identified by measuring the similarity between the samples and the known classes \cite{bendale2015towards, junior2017nearest}.
Scheirer \etal \cite{scheirer2013toward} applied the support vector machine (SVM) for known-class identification and adopted the extreme value distribution to detect the unknowns. Bendale \etal \cite{bendale2015towards} detected samples of unknown classes by calculating the similarity between the samples and the centroids of every known class, while J\'unior \etal \cite{junior2017nearest} considered the similarity between the most two similar classes. 

Recently, the powerful representation-learning capability of deep neural networks is used to detect unknowns. A plain choice is to make use of the maximum SoftMax probabilities and reject unconfident predictions \cite{hendrycks2016a}. However, Bendale \etal \cite{bendale2016towards} proved SoftMax probability is not robust and proposed to replace the SoftMax function with the OpenMax function, which redistributes the scores of Softmax to obtain the confident score of the unknown class explicitly. Ge \etal \cite{ge2017generative} proposed a G-Openmax method to further improve the Openmax by synthesizing samples of unknown classes based on the known-class samples. Neal \etal \cite{neal2018open} applied counterfactual image generation to augment fruitful samples for the unknown class. Zhang \etal \cite{zhang2020hybrid} proposed the OpenHybrid framework and utilize a flow-based density estimator to detect unknown samples. Zhou \etal \cite{zhou2021learning} raised the idea of placeholder learning where the overconfident predictions are calibrated by reserving classifier placeholders for unknown classes. Currently, AE-based methods and prototype-like methods are the most powerful ones, and a brief summary is made in the following.

\textbf{AE-based DNN Methods}.
%detect the unknowns based on the learned representation and reconstruction errors.
Zhang \etal \cite{zhang2017sparse} believed that the reconstruction errors contain useful discriminative information and proposed to leverage sparse representation to model the open set recognition problem.
Yoshihashi \etal \cite{yoshihashi2019classification} designed the CROSR method which uses latent representations for close-set classifier training and unknown detection. Oza and Patel \cite{oza2019c2ae} proposed a two-step C2AE method. It first trains the encoder for close-set identification, then keeps it fixed and adds the class-conditional information to train the decoder for unknown detection. Sun \etal \cite{sun2020conditional} used a variational auto-encoder to force different latent features to approximate different Gaussian models for unknown detection. This work is further extended to CPGM \cite{sun2020open}, which adds discriminative information into the probabilistic generative models. Perera \etal \cite{perera2020generative} feeds the raw and reconstructed image to a classification network, and the prediction is simultaneously confident when the reconstruction is consistent with raw input.

\textbf{Prototype-like DNN Methods}. Yang \etal \cite{prototype} proposed Generalized Convolutional Prototype Learning, which replaced close-world assumed softmax classifier with an open-world oriented prototype model. Chen \etal \cite{chen2020learning} developed Reciprocal Point Learning (RPL) that classifies a sample to known or unknown by the otherness with reciprocal points. Later, RPL is further improved to ARPL \cite{chen2021adversarial}, integrating an extra adversarial training strategy to enhance the model distinguishability to the known and unknown classes by generating confusing training samples.

\subsection{Out-of-Distribution Detection}
As is firstly introduced in \cite{hendrycks2016a}, OOD detection is to detect samples that do not belong to the training set. Several methods consider the problem where OOD samples are available during training \cite{lee2018a,liang2018enhancing,dhamija2018reducing,liu2020energy,quintanilha2018detecting,zisselman2020deep}. However, this does not meet our task where only in-distribution data is accessible during training. In the following, we mainly focus on models trained without extra OOD data.

\textbf{Supervised Methods.} With similar problem setting to open set recognition, these methods build OOD detectors upon a classification task. Some methods seek better score functions, including maximum SoftMax probability \cite{hendrycks2016a}, maximum logit scores \cite{hendrycks2019a}, and energy score \cite{liu2020energy}. Vyas \etal \cite{vyas2018out} used an ensemble of leave-one-out classifiers to simulate OOD accessible training individually. \cite{sastry2020detecting} proposed to characterize activity patterns with Gram matrices and score OOD-ness by calculating the element-wise deviation comparing to the Gram matrices from training data.

\textbf{Self-Supervised Methods.} These methods are relatively novel and take the advantage of the well-learned representations by self-supervision. \cite{hendrycks2019using,golan2018deep} consider the task of predicting image transformations (\eg rotating image $0\degree,90\degree,180\degree,270\degree$), which is also leveraged as an auxiliary task in \cite{tack2020csi}. Self-supervised contrastive learning has shown great success in unsupervised representation learning \cite{chen2020a,grill2020bootstrap}, and is also being applied for OOD detection \cite{tack2020csi,winkens2020contrastive,sehwag2021ssd}. They observed representations obtained by contrastive learning have distinct patterns between in- and out-distribution data. Though designed for unlabeled settings, these methods are also extended for supervised learning.
